Ordered Tree-Pushdown Systems

We define a new class of pushdown systems where the pushdown is a tree instead of a word. We allow a limited form of lookahead on the pushdown conforming to a certain ordering restriction, and we show that the resulting class enjoys a decidable reachability problem. This follows from a preservation of recognizability result for the backward reachability relation of such systems. As an application, we show that our simple model can encode several formalisms generalizing pushdown systems, such as ordered multi-pushdown systems, annotated higher-order pushdown systems, the Krivine machine, and ordered annotated multi-pushdown systems. In each case, our procedure yields tight complexity.

==> apds_rules.tex <==

% The annotation has always order n

\begin{align}
	\tag*{$(\pop k)$}
	\label{rule:popk}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
		\node {$a(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$b(k)$}
				child { node {$\var y_1$}}
				child { node {$\cdots$} edge from parent[draw=none]}
				child { node {$\var y_k$}}
				child { node {$\var y$}}
				}
		    child{ node {$\var x_{k+1}$} }
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
		    child{ node {$\var x$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$b(n)$}
			child{ node {$\var y_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var y_k$}}
		    child{ node {$\var x_{k+1}$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
		    child{ node {$\var y$}};
	\end{tikzpicture}
	\\
	\tag*{$(\push k {})$}
	\label{rule:pushk}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$a(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
		    child{ node {$\var x$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
		\node {$a(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$a(k)$}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none]}
				child{ node {$\var x_k$}}
			    child{ node {$\var x$}}
			}
			child{ node {$\var x_{k+1}$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
		    child{ node {$\var x$}};
	\end{tikzpicture}
	\\
	\tag*{$(\collapse)$}
	\label{rule:collapse}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$a(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
			child{ node {$b(n)$}
				child { node {$\var y_1$}}
				child { node {$\cdots$} edge from parent[draw=none]}
				child { node {$\var y_n$}}
				child { node {$\var y$}}
			};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
		\node {$b(n)$}
			child{ node {$\var y_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var y_n$}}
		    child{ node {$\var y$}};
	\end{tikzpicture}
	\\
	\tag*{$(\push {} b)$}
	\label{rule:pushb}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$a(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
		    child{ node {$\var x$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$b(n)$}
			child{ node {$a(1)$}
				child { node {$\var x_1$}}
				child { node {$\var x$}}
			}
			child{ node {$\var x_2$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
		    child{ node {$\var x_n$}}
			child{ node {$a(n)$}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none]}
			    child{ node {$\var x_n$}}
			    child{ node {$\var x$}}
			};
	\end{tikzpicture}
	\\
	\tag*{$(\rew b)$}
	\label{rule:rewb}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$a(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var x_n$}}
		    child{ node {$\var x$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$b(n)$}
			child{ node {$\var x_1$}}
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var x_n$}}
		    child{ node {$\var x$}};
	\end{tikzpicture}
\end{align}

\ignore{
\begin{align*}
\mathrm{\hat{\it pop}}_k:\quad		&	a(n)\ \var x\, \var x_1 \dots (b(k)\ \var y\, \var y_1 \dots \var y_k) \var x_{k+1} \dots \var x_n
							\goesto	b(n)\ \var y\, \var y_1 \dots \var y_k \var x_{k+1} \dots \var x_n \\
\mathrm{\hat{\it push}}_k:\quad		&	a(n)\ \var x\, \var x_1 \dots \var x_n
							\goesto	a(n)\ \var x\, \var x_1 \dots (a(k)\ \var x\, \var x_1 \dots \var x_k) \var x_{k+1} \dots \var x_n \\
\mathrm{\hat{\it collapse}}_k:\quad	&	a(n)\ (b(k)\ \var y\, \var y_1 \dots \var y_k) \var x_1 \dots \var x_n
							\goesto	b(n)\ \var y\, \var y_1 \dots \var y_k \var x_{k+1} \dots \var x_n \\
\mathrm{\hat{\it push}}^k_b:\quad 	&	a(n)\ \var x\, \var x_1 \dots \var x_n
							\goesto	b(n)\ \var x_k (a(1)\ \var x\, \var x_1) \var x_2 \dots \var x_n \\
\mathrm{\hat{\it rew_b}}:\quad 		&	a(n)\ \var x\, \var x_1 \dots \var x_n
							\goesto	b(n)\ \var x\, \var x_1 \dots \var x_n
\end{align*}
%
}

\ignore{

	% Previous rules where the annotation has arbitrary order k

	\begin{align}
		\tag*{(pop$\mbox{}_k$)}
		\label{rule:popk}
		&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
			\node {$a(n)$}
			    child{ node {$\var x$}}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
				child{ node {$b(k)$}
					child { node {$\var y$}}
					child { node {$\var y_1$}}
					child { node {$\cdots$} edge from parent[draw=none]}
					child { node {$\var y_k$}}
					}
			    child{ node {$\var x_{k+1}$} }
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\longgoesto
		\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$b(n)$}
			    child{ node {$\var y$}}
				child{ node {$\var y_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
				child{ node {$\var y_k$}}
			    child{ node {$\var x_{k+1}$} }
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\\
		\tag*{(push$\mbox{}_k$)}
		\label{rule:pushk}
		&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$a(n)$}
			    child{ node {$\var x$}}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\longgoesto
		\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
			\node {$a(n)$}
			    child{ node {$\var x$}}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
				child{ node {$a(k)$}
				    child{ node {$\var x$}}
					child{ node {$\var x_1$}}
				    child{ node {$\cdots$} edge from parent[draw=none] }
					child{ node {$\var x_k$}}
				}
				child{ node {$\var x_{k+1}$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\\
		\tag*{(collapse$\mbox{}_k$)}
		\label{rule:collapsek}
		&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$a(n)$}
				child{ node {$b(k)$}
					child { node {$\var y$}}
					child { node {$\var y_1$}}
					child { node {$\cdots$} edge from parent[draw=none]}
					child { node {$\var y_k$}}
				}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\longgoesto
		\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
			\node {$b(n)$}
			    child{ node {$\var y$}}
				child{ node {$\var y_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
				child{ node {$\var y_k$}}
			    child{ node {$\var x_{k+1}$} }
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\\
		\tag*{(push$\mbox{}_k^b$)}
		\label{rule:pushb}
		&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$a(n)$}
			    child{ node {$\var x$}}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\longgoesto
		\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$b(n)$}
				child{ node {$\var x_k$}}
				child{ node {$a(1)$}
					child { node {$\var x$}}
					child { node {$\var x_1$}}
				}
				child{ node {$\var x_2$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\\
		\tag*{(rew$\mbox{}^b$)}
		\label{rule:rewb}
		&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$a(n)$}
			    child{ node {$\var x$}}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
		\longgoesto
		\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
			\node {$b(n)$}
			    child{ node {$\var x$}}
				child{ node {$\var x_1$}}
			    child{ node {$\cdots$} edge from parent[draw=none] }
			    child{ node {$\var x_n$} };
		\end{tikzpicture}
	\end{align}
}


==> defs.tex <==
% General commands and notation
\newcommand{\ignore}[1]{}
\newcommand{\ifcont}[1]{}

\makeatletter
\newcommand{\@abbrev}[3]{
  \def\c@a@def##1{
      \if ##1.
        \relax
      \else
        \@ifdefinable{\@nameuse{#1##1}}{\@namedef{#1##1}{#2##1}}
        \expandafter\c@a@def
      \fi
    }
  \c@a@def #3.
}

\@abbrev{cal}{\mathcal}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}

%\newcommand{\ord}{\mathsf{ord}}
\newcommand{\deep}{\mathsf{deep}}
%\newcommand{\rank}{\mathsf{rank}}
%\newcommand{\sub}{\mathsf{sub}}
\newcommand{\encP}{\mathsf{enc}}
\newcommand{\Enc}{\mathsf{Enc}}
%\newcommand{\Nat}{\mathbb{N}}
%\newcommand{\br}[1]{\llbracket #1\rrbracket}

\changenotsign

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}

\newtheorem{proposition}{Proposition}

\renewcommand{\paragraph}{\subparagraph}

\newcommand{\Rpos}{\ensuremath{\mathbb{R}_{\geq 0}}}
\newcommand{\Nat}[0]{\ensuremath{\mathbb{N}}}
\newcommand{\Natpos}[0]{\ensuremath{\mathbb{N}_{>0}}}

\newcommand{\nexp}[2]{\mathsf{exp}_{#1}({#2})}

\newcommand{\ptime}{$\mathsf{PTIME}$\xspace}
\newcommand{\twoexptimec}{$\mathsf{2\textrm-EXPTIMEc}$\xspace}
\newcommand{\twoexptimeh}{$\mathsf{2\textrm-EXPTIME}$-hard\xspace}
\newcommand{\exptime}{$\mathsf{EXPTIME}$\xspace}
\newcommand{\exptimec}{$\mathsf{EXPTIMEc}$\xspace}
\newcommand{\exptimeh}{$\mathsf{EXPTIME}$-hard\xspace}
\newcommand{\nexptimec}[1]{$\mathsf{{#1}\textrm-EXPTIMEc}$\xspace}
\newcommand{\nexptimeh}[1]{$\mathsf{{#1}\textrm-EXPTIME}$-hard\xspace}
\newcommand{\nexptime}[1]{$\mathsf{{#1}\textrm-EXPTIME}$\xspace}

\newcommand{\lambdaY}{$\lambda Y$}

\renewcommand{\st}{\ |\ }
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\setof}[2]{\set{#1 \st #2}}
\newcommand{\SetOf}[2]{\left\{{#1} \left.\right| #2\right\}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
%\newcommand{\smaller}{\prec}
\newcommand{\proj}[2]{\left.{#1}\right|_{#2}}
\newcommand{\var}[1]{\mathsf{#1}}
\newcommand{\varord}[3]{\mathsf{#1}_{#2}^{#3}}
\newcommand{\Vars}{\mathcal{V}}
\newcommand{\vars}[1]{\Vars(#1)}
\newcommand{\freevars}[1]{\mathsf{FV}(#1)}
\newcommand{\pos}[1]{\mathsf{pos}(#1)}
\newcommand{\Trees}[1]{\mathcal{T}({#1})}
\newcommand{\sem}[1]{\llbracket#1\rrbracket}
\newcommand{\model}[1]{\mathcal #1}
\newcommand{\BT}[1]{BT(#1)}
\newcommand{\frontier}[2]{\mathsf{frontier}(#1, #2)}
\newcommand{\Rules}{\mathcal{R}}
\newcommand{\ShallowRules}{\mathcal R_{\textrm s}}
\newcommand{\DeepRules}{\mathcal R_{\textrm d}}
\newcommand{\pow}[1]{2^{#1}}
\def\rddots#1{\cdot^{\cdot^{\cdot^{#1}}}}
\newcommand{\Closures}{Cl}
\newcommand{\context}[1]{\mathsf{context}({#1})}
\newcommand{\width}[1]{\mathsf{width}({#1})}

\newcommand{\marked}[1]{[#1]}

\newcommand{\proves}{\vdash}
\newcommand{\arrow}{\to}
\newcommand{\oftype}{\coloncolon}
\newcommand{\ofrank}{\colon} %{\coloncolon}

\newcommand{\recscheme}[1]{\mathcal R}

\newcommand{\pds}{\mathcal P}
\newcommand{\ATA}{\mathcal}
\newcommand{\loc}{\ell}
\newcommand{\project}{\mathsf{proj}}
\newcommand{\cpy}{\mathsf{copy}}
\newcommand{\rank}{\mathsf{rank}}
\newcommand{\ord}{\mathsf{ord}}
\newcommand{\level}[1]{\mathsf{level}({#1})}

\newcommand{\goesto}{\rightarrow}
\newcommand{\rewritesto}{\rightarrow}
\newcommand{\longgoesto}{\longrightarrow}
\newcommand{\goestostar}{\rightarrow^*}
\newcommand{\replacedby}{\mapsto}
\newcommand{\reads}[1]{\,\textrm{---}#1\goesto}
\newcommand{\trans}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\reaches}[1]{\stackrel{#1}{\rightsquigarrow}}
\newcommand{\notreaches}[1]{{{\stackrel{#1}{\not\rightsquigarrow}}}}

\newcommand{\prename}{\mathrm{Pre}}
\newcommand{\pre}[1]{\prename({#1})}
\newcommand{\prestarname}{\prename^*}
\newcommand{\prestar}[1]{\prestarname({#1})}

\newcommand{\lang}[1]{\mathcal L({#1})}

\newcommand{\totree}[1]{\mathcal T(#1)}

\newcommand{\Sys}{\mathcal S}
\newcommand{\OMPDS}{\mathcal O}
\newcommand{\APDS}{\mathcal P}
\newcommand{\KM}{\mathcal M}
\newcommand{\OAMPDS}{\mathcal R}

\newcommand{\ihat}{{\hat \imath}}
\newcommand{\cc}{\mathtt{cc}}
\newcommand{\cont}{\mathrm{cont}}

\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\when}{\leftarrow}
\newcommand{\size}[1]{\left|{#1}\right|}
%\newcommand{\restrict}[2]{{#1}_{|#2}}
\newcommand{\restrict}[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}

\newcommand{\stack}[1]{\langle{#1}\rangle}
\newcommand{\enc}[2]{\mathsf{enc}_{#1}({#2})}
\newcommand{\encB}[2]{\mathsf{enc}^\bullet_{#1}({#2})}
\newcommand{\dec}[2]{\mathsf{dec}_{#1}({#2})}
\newcommand{\tenc}[2]{\mathsf{tenc}_{#1}({#2})}
\newcommand{\tdec}[2]{\mathsf{tdec}_{#1}({#2})}

% operations for ordered tree-pushdown systems
\newcommand{\pop}{\mathsf{pop}}
\newcommand{\push}{\mathsf{push}}
\newcommand{\scan}{\mathsf{scan}}
\newcommand{\pushp}{\mathsf{push'}}
\newcommand{\scanp}{\mathsf{scan'}}
\newcommand{\scanpop}{\mathsf{scan\textrm-pop}}

% operations for ordered multi-pushdown systems
\newcommand{\opop}[2]{\pop_{#1}({#2})}
\newcommand{\opush}[2]{\push_{#1}({#2})}

% operations for annotated pushdown systems
\newcommand{\collapse}{\mathsf{collapse}}
\newcommand{\apop}[1]{\pop_{#1}}
\newcommand{\apush}[2]{\push_{#1}^{#2}}
\newcommand{\acollapse}[1]{\collapse_{#1}}
\newcommand{\apoparg}[2]{\apop {#1} ({#2})}
\newcommand{\apusharg}[3]{\apush {#1} {#2} ({#3})}
\newcommand{\acollapsearg}[2]{\acollapse {#1} ({#2})}
%\newcommand{\rew}[1]{\mathsf{rew}_{#1}}
%\newcommand{\hpop}[1]{\hat{\mathsf{pop}}_{#1}}
%\newcommand{\hpush}[2]{\hat{\mathsf{push}}_{#1}^{#2}}
%\newcommand{\hcollapse}{\hat{\mathsf{collapse}}}
%\newcommand{\hrew}[1]{\hat{\mathsf{rew}}_{#1}}

\newcommand{\dollar}{\$}

%\newenvironment{apptheorem}[1]
%	{\noindent\textcolor{darkgray}{$\blacktriangleright$}\nobreakspace{\sffamily\bfseries Theorem~\ref{#1}.}\it}
%	{}
	
\newenvironment{shortproof}
	{\begin{proof}[Proof idea]}
	{\end{proof}}

% Todo commands
\newcommand{\lorenzo}[1]{\todo[color=yellow]{#1}}
\newcommand{\igw}[1]{\todo[color=green]{#1}}
\newcommand{\pppp}[1]{\todo[color=red]{#1}}

% For repeating theorems and lemmas in appendix
%\newcommand{\Repeat}[2]{\noindent{$\blacktriangleright$\textsc{\textbf{#1~\ref{#2}.\
 %     }}}}

% Vectors, taken from llncs.cls
\def\vec#1{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}


==> fig_saturation.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		
		\draw (0, 0) -- (4, 0);
		\draw[dashed] (4, 0) -- (7, 0);
		\draw (0, 0) -- (0, 5);
		\draw (4, 0) -- (3, 3);
		\draw (0, 3) -- (3, 3);
		\draw (3, 3) -- (3, 5);
		\draw (0, 5) -- (3, 5);
		\draw[dashed] (3, 3) -- (7, 3);
		\draw[dashed] (7, 0) -- (7, 3);
		
		\node at (.5, 4.5) {$P_E$};
		\node at (.5, .5) {$P_C$};
		\node at (6.2, .5) {$Q_C \setminus P_C$};
		
		\node [text width = 1cm] (p) at (1.5, 3.5) {\ } edge [in=30,out=120,loop] node [above] {$f$} ();
		\node [text width = 1cm] (q) at (1, 1.5) {\ } edge [in=-30,out=-120,loop] node [below] {$M$} ();
		\node [text width = 1cm] (q') at (2, 1.5) {\ };
		\node [text width = 1cm] (p') at (5, 1) {\ } edge [in=-30,out=60,loop,dashed,double] node [above right] {$M$} ();
		%	{$\begin{array}{c}M\\\textrm{(by \ref{eq:rule:lift})}\end{array}$} ();
		
		\path[->] (p) edge [bend right] node [left] {$[M]$} (q);
		\path[->, dashed] (p) edge [bend left] node [above right, pos = .7] {$[M]$} (q');
		\path[->, dashed] (p) edge [bend left] node [above right, pos = .3] {$[M]$} (p');
		\path[->, dashed] (p') edge [double, bend right] node [above] {$M$} (q');
		%node [below] {(by \ref{eq:rule:lift})} 
		
	\end{tikzpicture}
	\caption{Illustration of the states and transitions added by the saturation procedure (dashed).}
	\label{fig:saturation}
\end{figure}

==> km_rules.tex <==
\begin{align}
	\tag*{(var)}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked x$}
		    child{ node {$M$}
				child { node {$\var x_1$} }
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_n$} } }
			child{ node {$\var y_1$} }
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var y_k$} };
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked M$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child{ node {$\var y_1$} }
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var y_k$} };
	\end{tikzpicture}
	\\
	\tag*{(app)}
	\label{rule:app}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked {M N}$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child{ node {$\var y_1$} }
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var y_k$} };
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
		\node {$\marked M$}
		  	child { node {$\var x_{i_1}$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_{i_{n_0}}$} }
			child{ node {$N$}
				child { node {$\var x_{j_1}$} }
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_{j_{n_1}}$} } }
			child{ node {$\var y_1$} }
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var y_k$} };
	\end{tikzpicture}
	\\
	\tag*{(fix)}
	\label{rule:fix}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked {Y M}$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child{ node {$\var y_1$} }
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var y_k$} };
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.5cm}]
		\node {$\marked M$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child{ node {$Y M$}
				child { node {$\var x_1$} }
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_n$} } }
			child{ node {$\var y_1$} }
		    child{ node {$\cdots$} edge from parent[draw=none] }
		    child{ node {$\var y_k$} };
	\end{tikzpicture}
	\\
	\tag*{(abs$\mbox{}_1$)}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked {\lambda x \cdot M}$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child { node {$\var y_0$} }
			child { node {$\var y_1$} }
		    child { node {$\cdots$} edge from parent[draw=none] }
		    child { node {$\var y_k$} };
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked M$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var y_0$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child { node {$\var y_1$} }
		    child { node {$\cdots$} edge from parent[draw=none] }
		    child { node {$\var y_k$} };
	\end{tikzpicture}
	&&\textrm{ if $x$ is free in $M$ }
	\\
	\tag*{(abs$\mbox{}_2$)}
	\label{rule:abs2}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked {\lambda x \cdot M}$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child { node {$\var y_0$} }
			child { node {$\var y_1$} }
		    child { node {$\cdots$} edge from parent[draw=none] }
		    child { node {$\var y_k$} };
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.2cm}]
		\node {$\marked M$}
		  	child { node {$\var x_1$} }
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\var x_n$} }
			child { node {$\var y_1$} }
		    child { node {$\cdots$} edge from parent[draw=none] }
		    child { node {$\var y_k$} };
	\end{tikzpicture}
	&&\textrm{ if $x$ is not free in $M$ }
	\\
	\tag*{(const)}
	&\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 2.2cm/#1}]
		\node {$\marked f$}
		  	child { node {$M_1$}
				child { node {$\var x_{11}$}}
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_{1n_1}$}}
				}
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$M_k$}
				child { node {$\var x_{k1}$}}
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_{kn_k}$}}}
			;
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 2.2cm/#1}]
		\node {$f$}
		  	child { node {$\marked {M_1}$}
				child { node {$\var x_{11}$}}
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_{1n_1}$}}
				}
			child { node {$\cdots$} edge from parent[draw=none] }
			child { node {$\marked {M_k}$}
				child { node {$\var x_{k1}$}}
				child { node {$\cdots$} edge from parent[draw=none] }
				child { node {$\var x_{kn_k}$}}}
			;
	\end{tikzpicture}
	%&&\textrm{ for every } P \trans f Q_1 \dots Q_k
\end{align}

==> ompds_rules.tex <==

\begin{align}
	\tag*{$(\pop 1)$}
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$a(k)$}
			child{ node {$b$} child { node {$\var x_k$}}}
			child{ node {$\var x_{k+1}$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$b(k)$}
			child{ node {$\var x_k$}}
			child{ node {$\var x_{k+1}$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\\
	\tag*{$(\pop 2)$}
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$a(k)$}
			child{ node {$\bot$}}
			child{ node {$b$} child {node {$\var x_{k+1}$}}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$b(k+1)$}
			child{ node {$\var x_{k+1}$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\\
	\tag*{$(\push b {h \leq k})$}
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$a(k)$}
			child{ node {$\var x_k$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$b(h)$}
			child{ node {$\bot$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\bot$}}
			child{ node {$a$} child {node {$\var x_k$}}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\\
	\tag*{$(\push b {h > k})$}
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$a(k)$}
			child{ node {$\var x_k$}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
	\longgoesto
	\begin{tikzpicture}[baseline=-2.3ex,scale=0.5,level/.style={sibling distance = 1.4cm}]
		\node {$a(k)$}
			child{ node {$\var x_k$}}
			child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$b$} child {node {$\var x_h$}}}
		    child{ node {$\cdots$} edge from parent[draw=none]}
			child{ node {$\var x_n$}};
	\end{tikzpicture}
\end{align}

==> pds.tex <==

\subsection{Pushdown systems}

An \emph{alternating pushdown system} is a tuple $\pds = \tuple {\Gamma, Q, q_0, F, \Delta}$
where $\Gamma$ is a finite pushdown alphabet,
$Q$ is a finite set of control locations,
$q_0$ is the initial control location,
$F \subseteq Q$ is the set of accepting locations,
and $\Delta$ is a finite set of transition rules of the form
$(p, \alpha) \goesto (P, \varepsilon)$ (pop)
and $(p, \alpha) \goesto (P, \beta\gamma)$ (push),
where $p\in Q$, $P \subseteq Q$, and $\alpha, \beta, \gamma \in \Gamma$.
%
We say that $\pds$ is \emph{non-deterministic} if $P$ is a singleton for every rule.
%
\lorenzo{define configurations and formally state simulation?}

\lorenzo{complete the def. below}
%
It is immediate to associate to a pushdown system $\pds$ as above
a unary AOTPS with states $\Sys = \tuple {\Sigma, Q, \Rules}$.
The idea is to encode a pushdown $w$ as a linear tree in the obvious way.
Thus, we take $\Sigma = \Gamma \cup \set{\bot}$ as an ordered alphabet
where symbols in $\Gamma$ have rank $1$ and $\bot$ is a new symbol not in $\Gamma$ of rank $0$.
Since all symbols have rank at most $1$, the order is irrelevant.
This is further reinforced by the fact that we do not use scan rules.
Formally, one can assume that all symbols in $\Sigma$ and variables have order $1$.
For each pop rule $(p, \alpha) \goesto (P, \varepsilon)$ in $\Delta$,
there is the following pop rule in $\Rules$:
%
\begin{align}
	\label{rule:PDS:pop}
	p, \begin{tikzpicture}[baseline=-.5ex,scale=0.5]
		\node {$\alpha$}
			child { node {$\var x$}};
	\end{tikzpicture}
	\longgoesto
	P, \var x
\end{align}
%
For each push rule $(p, \alpha) \goesto (P, \beta\gamma)$ in $\Delta$,
there is the following push rule in $\Rules$:
%
\begin{align}
	\label{rule:PDS:push}
	p, \begin{tikzpicture}[baseline=-.5ex,scale=0.5]
		\node {$\alpha$}
			child { node {$\var x$}};
	\end{tikzpicture}
	\longgoesto
	P, \begin{tikzpicture}[baseline=-.5ex,scale=0.5]
		\node {$\beta$}
			child{ node {$\gamma$}
				child{ node {$\var x$}}};
	\end{tikzpicture}
\end{align}
%
Here, the variable $\var x$ has order $0$.
It is immediate to see that the rules above satisfies the constraints~\ref{enum:I} and \ref{enum:II} of AOTPSs.

\begin{remark}[Complexity]
	%
	Since we construct a unary AOTPS,
	by Remark~\ref{rem:size:delta':unary} the saturation procedure has polynomial complexity if both $\pds$ and $\ATA A$ are non-deterministic,
	and exponential complexity otherwise.
	%$\size {\Delta'} \leq O(\size {\mathcal R} \cdot {\size {Q'}}^r) = O(\size {\mathcal R} \cdot {\size Q}^r)$.
	%This is made possible by the fact that we use control locations in the ordered tree-pushdown system.
	%However, control locations can be dispensed with if the scan operation is available,
	%as discussed in Remark~\ref{rem:states}.
\end{remark}

